RASSAR: Room Accessibility and Safety Scanning in Augmented Reality

The safety and accessibility of our homes is critical to quality of life and evolves as we age, become ill, host guests, or experience life events such as having children. Researchers and health professionals have created assessment instruments such as checklists that enable homeowners and trained experts to identify and mitigate safety and access issues. With advances in computer vision, augmented reality (AR), and mobile sensors, new approaches are now possible. We introduce RASSAR, a mobile AR application for semi-automatically identifying, localizing, and visualizing indoor accessibility and safety issues such as an inaccessible table height or unsafe loose rugs using LiDAR and real-time computer vision. We present findings from three studies: a formative study with 18 participants across five stakeholder groups to inform the design of RASSAR, a technical performance evaluation across ten homes demonstrating state-of-the-art performance, and a user study with six stakeholders. We close with a discussion of future AI-based indoor accessibility assessment tools, RASSAR's extensibility, and key application scenarios.

==> Tables/Demographics.tex <==
\begin{table}[htb!]
\centering
\label{table:demographics}
\caption{Our formative study included 18 participants. PID stands for Participant Index. Older Adults refers to those aged 65 and over. Children refers to those between 0 and 3 years old. BLV refers to people who are blind or low vision. OT refers to occupational therapists. "Caregiver" means the participant is a caregiver, not a member, of the community.}
 \renewcommand{\arraystretch}{1.05}
    \begin{tabular}{lcllll}
    \hline
    \makecell[c]{PID} & \makecell[c]{Wheelchair \\ User} & \makecell[c]{Older \\ Adults} & Children & BLV & OT \\ \hline
    P1 & Yes & No & No & No & No\\
    P2 & Yes & No & No & No & No\\
    P3 & Yes & No & No & No & No\\
    P4 & Yes & No & No & No & No\\
    P5 & Yes & No & No & No & No\\
    P6 & Yes & No & No & No & No\\
    P7 & No & No & Caregiver & No & No\\
    P8 & Yes & Yes & No & No & No\\
    P9 & No & Caregiver& Caregiver & No & No\\
    P10& Yes & Yes & No & No & No\\
    P11& No & No & No & No & Yes \\
    P12& No & No & No & No & Yes \\
    P13& No & Yes & No & Yes& No\\
    P14& No & Yes & No & Yes& No\\
    P15& No & Yes & No & Yes& No\\
    P16& No & No & Caregiver & No & No\\
    P17& No & No & No & No & Yes \\
    P18& No & No & No & Yes& No\\ \hline
    \end{tabular}
    \label{tab:demographics}
\end{table}

==> Tables/EvaluationResults.tex <==
\begin{table*}[htb!]
    \centering
    \caption{Evaluation Results. GT refers to ground truth obtained from the RASSAR accessibility rubrics. Scanning time was measured in seconds.}
    % Items labeled as  are calculated based on GT-20, while items labeled as \ding{70} are calculated based on GT-HASSAT. }
  \label{tab:evaluationresults}
  \resizebox{0.85\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|r|r|r|r|r|r|r}\hline
    \makecell[c]{Space \\ ID} & \makecell[c]{Count \\ of GT}  & \makecell[c]{Count \\ of Scan Results} & \makecell[c]{Count \\ of TP} & \makecell[c]{Count \\ of FP} & \makecell[c]{Count \\ of FN} &  \makecell[c]{Precision} & Recall & F1 Score & Accuracy & \makecell[c]{Fleiss' \\ Kappa} & \makecell[c]{Scanning \\ Time} \\\hline
    \multirow{3}{*}{S1} & \multirow{3}{*}{15}  & 20 & 14 & 5 & 1  & 0.737 & 0.933 & 0.824 & 0.700 & \multirow{3}{*}{0.726} &  \multirow{3}{*}{113 seconds} \\\cline{3-10} 
    &  &  20 & 13 & 5 & 2  & 0.722 & 0.867 & 0.788 & 0.650 &  &  \\\cline{3-10} 
    &  &  19 & 14 & 4 & 1  & 0.778 & 0.933 & 0.848 & 0.737 &  &   \\\hline
    \multirow{3}{*}{S2} & \multirow{3}{*}{11} &  16 & 9 & 5 & 2  &0.643  &0.818  &0.720  &0.563  &  \multirow{3}{*}{0.694} &  \multirow{3}{*}{120 seconds}\\\cline{3-10} 
    &  &  14  &8& 3 &3  & 0.727& 0.727&0.727  &0.571  &  & \\\cline{3-10} 
    &  &    13& 7 &2 & 4 &0.778  &0.636  &0.700  &0.538  &  & \\\hline
    \multirow{3}{*}{S3} & \multirow{3}{*}{24}   &30  &21  &6  &3   &0.778  &0.875  &0.824  &0.700  &  \multirow{3}{*}{0.495} &  \multirow{3}{*}{148 seconds}\\\cline{3-10} 
    &  &   28 &  18&  4&  6 & 0.818 & 0.750 & 0.783 & 0.727 & & \\\cline{3-10} 
    &  &  25 & 18 & 1 & 6 & 0.947 & 0.750&  0.837&  0.643&  &  \\\hline
    \multirow{3}{*}{S4} & \multirow{3}{*}{11} & 12 & 8 & 1 & 3 & 0.889 & 0.727 & 0.800 & 0.667 & \multirow{3}{*}{1.000} &   \multirow{3}{*}{80 seconds}\\\cline{3-10} 
    &  &  11 & 9 & 0 & 2 & 1.000 & 0.818 & 0.900 & 0.818 &  &  \\\cline{3-10} 
    &  &  13 & 9 & 2 & 2  & 0.818 & 0.818 & 0.818 & 0.692 &  &  \\\hline
    \multirow{3}{*}{S5} & \multirow{3}{*}{11} & 12 & 10 & 1 & 1 & 0.909 & 0.909 & 0.909 & 0.833 & \multirow{3}{*}{1.000} & \multirow{3}{*}{84 seconds}  \\\cline{3-10} 
    &  &  12 & 10 & 1 & 1  & 0.909 & 0.909 & 0.909 & 0.833 &  &  \\\cline{3-10} 
    &  &   11&  10&  0&  1&  1.000 &  0.909&  0.952&  0.909&  &  \\\hline
    \multirow{3}{*}{S6} &\multirow{3}{*}{13}  &  14&  11&  1&  2&   0.917& 0.846 & 0.880 & 0.786 & \multirow{3}{*}{0.826} & \multirow{3}{*}{125 seconds} \\\cline{3-10} 
    &  &  15&  11&  2&  2&   0.846&  0.846&  0.846&  0.733& & \\\cline{3-10} 
    &  &  13 & 10 & 0 & 3  & 1.000 & 0.769 & 0.846 & 0.733 &  & \\\hline
    \multirow{3}{*}{S7} &\multirow{3}{*}{15} & 19 & 13 & 4 & 2 & 0.765 & 0.867 & 0.813 & 0.684 & \multirow{3}{*}{0.615} & \multirow{3}{*}{96 seconds} \\\cline{3-10} 
    &  &  18 & 13 & 3 & 2  &  0.813&  0.867&  0.839&  0.722&  &  \\\cline{3-10} 
    &  &   16&  13&  1&  2&  0.929&  0.867&  0.897&  0.722&  &  \\\hline
    \multirow{3}{*}{S8} & \multirow{3}{*}{10} & 10 & 7 & 0 & 3  & 1.000 & 0.700 & 0.824 & 0.700 & \multirow{3}{*}{0.683} &  \multirow{3}{*}{80 seconds} \\\cline{3-10} 
    &  &  10 & 6 & 0 & 4 & 1.000 & 0.600 & 0.75 & 0.600 &  &  \\\cline{3-10} 
    &  &  10 & 8 & 0 & 2 & 1.000 & 0.800 & 0.889 & 0.800 &  &  \\     \hline
    \end{tabular}}
\end{table*}


==> Tables/Json.tex <==
% \renewcommand{\arraystretch}{1.2}
% \begin{table*}[htb!]
% \centering
% \caption{The JSON elements and their values in our input specification file}
%   \label{tab:json}
% \begin{tabular}{C{0.15\textwidth} L{0.28\textwidth} L{0.1\textwidth} C{0.09\textwidth} L{0.8\textwidth}}
% \hline
% \textbf{JSON Element} & \textbf{Description}                                                                                              & \multicolumn{3}{l}{\textbf{Values}}                                                                                                                                                               \\ \hline
% Object of interest    & The object to automatically identify. We currently support 18 objects.                                            & \multicolumn{3}{l}{\textit{Cabinet, chair, counter, door, door handle, electric socket, grab bar, knives, knob, light switch, medication, rug, sink, scissors, smoke alarm, sofa, table, toilet}} \\
% Rubric type           & What type of accessibility / safety issues are we trying to detect.                                               & \multicolumn{3}{l}{\textit{Dimensional Height, Positional Height and Existence}}                                                                                                                  \\
% Community             & The impacted target group(s)                                                                                      & \multicolumn{3}{l}{\textit{Children, older adults, blind or low vision, wheelchair users. Can select one or more.}}                                                                               \\
% Dependency            & Relational dependence (if any)                                                                                    & \multicolumn{3}{l}{Can specify any Object of interest. E.g. toilet.}                                                                                                                              \\
% Dimension             & Specifies dimensional requirements and conditional logic (e.g., a door must be a minimum of 32” wide)             & \multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}Comparators like greater than, less than, between or equal.\\ Values as one or two length values in inches.\end{tabular}}                           \\
% Existence             & Does the object pose a problem by its sheer existence at the location?                                            & \multicolumn{3}{l}{Can be null, true, or false. If null, then this Object of interest is not about existence but about dimension or position.}                                                    \\
% Description           & A human-readable description of the problem, which is drawn from existing ADA standards and assessment checklists & \multicolumn{3}{l}{Plain text}                                                                                                                                                                    \\
% Source                & A link to the original source of this certain accessibility rubric.                                               & \multicolumn{3}{l}{Source name as plain text and URL.}                                                                                                                                            \\
% Suggestion            & One or more human-readable suggestions to fix this certain issue.                                                 & \multicolumn{3}{l}{Plain text}                                                                                                                                                                    \\ \hline
% \end{tabular}
% \end{table*}

\renewcommand{\arraystretch}{1.05}
\begin{table*}[htb!]
\centering
\caption{The JSON elements and their values in our input specification file}
  \label{tab:json}
\resizebox{0.95\textwidth}{!}{\begin{tabular}{p{0.15\textwidth}p{0.3\textwidth}p{0.45\textwidth}}
\hline
\textbf{\makecell[c]{JSON Element}} & \textbf{\makecell[c]{Description}} & \textbf{\makecell[c]{Values}} \\\hline
Object of interest & The object to automatically identify. We currently support 18 objects. & Cabinet, chair, counter, door, door handle, electric socket, grab bar, knives, knob, light switch, medication, rug, sink, scissors, smoke alarm, sofa, table, toilet. \\\hline
Rubric type & What type of accessibility/safety issues are we trying to detect. & Dimensional Height, Positional Height and Existence. \\\hline
Community & The impacted target group(s) & Children, older adults, blind or low vision, wheelchair users. Can select one or more. \\\hline
Dependency & Relational dependence (if any). & Can specify any Object of interest. E.g. toilet. \\\hline
Dimension & Specifies dimensional requirements and conditional logic (e.g., a door must be a minimum of 32” wide). &  Comparators like greater than, less than, between, or equal. Values as one or two length values in inches. \\\hline
Existence & Does the object pose a problem by its sheer existence at the location? & Can be null, true, or false. If null, then this Object of interest is not about existence but about dimension or position. \\\hline
Description & A human-readable description of the problem, which is drawn from existing ADA standards and assessment checklists. &  Plain text. \\\hline
Source & A link to the original source of this certain accessibility rubric. & Source name as plain text and URL. \\\hline
Suggestion & One or more human-readable suggestions to fix this certain issue. & Plain text. \\\hline
\end{tabular}}
\end{table*}


==> Tables/PerformanceByIssue.tex <==
\begin{table*}[htb!]
\centering
\caption{Detection performance of different accessibility/safety issues. GT stands for ground truth from manual auditing. RP stands for RoomPlan. Acc is the abbreviation of accuracy.}
  \label{tab:performancebyissue}
   \resizebox{0.99\textwidth}{!}{
\begin{tabular}{|l|l|c|c|c|c|c|r|r|r|r|l|}\hline
Issue Name & Category & \makecell[c]{Total \\ Occurance\\ in GT} & \makecell[c]{Total \\ scan } & \makecell[c]{Count \\ of TP} & \makecell[c]{Count\\ of FP} & \makecell[c]{Count \\of FN} & \makecell[c]{\makecell[c]{Pre-\\cision}} & Recall & F1 & Acc & \makecell[c]{Main cause\\ of error} \\\hline
Counter Height          & \multirow{4}{*}{\makecell[l]{Object \\ Dimension }}               & 39  & 4    & 3     & 1     & 36    & 0.75    & 0.077& 0.14   & 0.075  & RP Misclassification              \\\cline{1-1}\cline{3-12}
table height            & & 33  & 35   & 30    & 5     & 3     & 0.857   & 0.909& 0.882  & 0.789  & RP Measurement                    \\\cline{1-1}\cline{3-12}
Door radius             &  & 21  & 16   & 13    & 3     & 8     & 0.813   & 0.619& 0.703  & 0.542  & RP Measurement                    \\\cline{1-1}\cline{3-12}
Bed Height              &  & 15  & 15   & 15    & 0     & 0     & 1       & 1    & 1      & 1      & -            \\\hline
Sink height             & \multirow{3}{*}{Object Position}                & 48  & 45   & 45    & 0     & 3     & 1       & 0.938& 0.968  & 0.938  & RP Miss     \\\cline{1-1}\cline{3-12}
Cabinet Height          &               & 42  & 42   & 42    & 0     & 0     & 1       & 1    & 1      & 1      &     -           \\\cline{1-1}\cline{3-12}
Grab bar height         &                 & 15  & 20   & 12    & 8     & 3     & 0.6     & 0.8  & 0.686  & 0.522  & YOLO Misclassification                  \\\hline
Rug                     & \multirow{4}{*}{\makecell[l]{Existence of \\ Risky Item}}      & 45  & 47   & 45    & 2     & 0     & 0.957   & 1    & 0.978  & 0.957  & YOLO Misclassification                  \\\cline{1-1}\cline{3-12}
Medication              &       & 15  & 30   & 13    & 17    & 2     & 0.433   & 0.867& 0.578  & 0.406  & YOLO Misclassification                  \\\cline{1-1}\cline{3-12}
Knife                   &       & 15  & 21   & 14    & 7     & 1     & 0.667   & 0.933& 0.778  & 0.636  & YOLO Misclassification                  \\\cline{1-1}\cline{3-12}
Scissors                &      & 9   & 9    & 9     & 0     & 0     & 1       & 1    & 1      & 1      &    -            \\\hline
No Grab bar near toilet & \multirow{2}{*}{\makecell[l]{Non-existence \\ of 
 Assistive Item}} & 21  & 18   & 18    & 0     & 3     & 1       & 0.857& 0.923  & 0.857  & YOLO Misclassification                  \\\cline{1-1}\cline{3-12}
No Grab bar near tub    &  & 12  & 10   & 10    & 0     & 2     & 1       & 0.833& 0.909  & 0.833  & YOLO Misclassification                  \\ \hline
\end{tabular}}
\end{table*}

==> Tables/Spaces.tex <==
\begin{table}[htb!]
\centering
\caption{Home spaces selected for technical evaluation}
  \label{tab:spaces}
  % \resizebox{0.45\textwidth}{!}{
\begin{tabular}{p{0.03\textwidth}p{0.15\textwidth}p{0.07\textwidth}p{0.15\textwidth}}
\hline
Index & Space Type          & Total Size & Space scanned                           \\ \hline
S1    & 1b1b apartment      & 670 sqf    & Kitchen, living room, bedroom, bathroom \\
S2    & 1b1b apartment      & 660 sqf    & Kitchen, living room, bathroom          \\
S3    & Single family house & 4000sqf    & Kitchen, living room, bedroom, bathroom \\
S4    & 2b2b apartment      & 600 sqf    & Kitchen, living room, bedroom, bathroom \\
S5    & 1b1b apartment      & 540 sqf    & Kitchen, living room, bedroom, bathroom \\
S6    & 2b2b apartment      & 1000 sqf   & Kitchen, living room, bedroom, bathroom \\
S7    & 1b1b apartment      & 670 sqf    & Kitchen, living room, bedroom, bathroom \\
S8    & Studio apartment    & 560 sqf    & Kitchen, living room, bedroom, bathroom \\ \hline
\end{tabular}
\end{table}
